HyperTuning: Toward Adapting Large Language Models without Back-propagation

Fine-tuning large language models for different tasks can be costly and inefficient, and even methods that reduce the number of tuned parameters still require full gradient-based optimization. We propose HyperTuning, a novel approach to model adaptation that uses a hypermodel to generate task-specific parameters for a fixed downstream model. We demonstrate a simple setup for hypertuning with HyperT5, a T5-based hypermodel that produces soft prefixes or LoRA parameters for a frozen T5 model from few-shot examples. We train HyperT5 in two stages: first, hyperpretraining with a modified conditional language modeling objective that trains a hypermodel to generate parameters; second, multi-task fine-tuning (MTF) on a large number of diverse language tasks. We evaluate HyperT5 on P3, MetaICL and Super-NaturalInstructions datasets, and show that it can effectively generate parameters for unseen tasks. Moreover, we show that using hypermodel-generated parameters as initializations for further parameter-efficient fine-tuning improves performance. HyperTuning can thus be a flexible and efficient way to leverage large language models for diverse downstream applications.

==> tables/table_05_natinst_em_rouge.tex <==
\begin{table}[th]
\parbox{.45\linewidth}{
    \centering
    \small
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrr}
        \toprule
         & AVG
    \\ \midrule
    \multicolumn{2}{l}{\textit{Full Fine-Tuning}} \\
    \ \ T5-MTF (Def) & 37.3
        \\
    \ \ T5-MTF (Def+2Pos) & 46.1
    \\ \midrule
    % \multicolumn{2}{l}{\textit{Parameter-Efficient Fine-Tuning (PEFT)}} \\
    % \ \ T5-MTF (Prefix)
    %     \\
    % \ \ T5-MTF (LoRA)
    % \\ \midrule
    \multicolumn{2}{l}{\textit{HyperTuning}} \\
    \ \ HyperT5-Prefix (Def) & 34.2
        \\
    \ \ HyperT5-Prefix (Def+2Pos) & 42.0
        \\
    \ \ HyperT5-LoRA (Def) & 30.9
        \\
    \ \ HyperT5-LoRA (Def+2Pos) & 40.2
        \\
        \bottomrule
    \end{tabular}%
    % }
    \caption{
        Results on Super-NaturalInstuctions (S-NI; Test) with T5-Large models.
    }
    \label{tab:table_04_natinst}
}
\parbox{.07\linewidth}{\ }
\parbox{.45\linewidth}{
    \centering
    \small
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrr}
        \toprule
         & AVG
    \\ \midrule
    \multicolumn{2}{l}{\textit{Full Fine-Tuning}} \\
    \ \ T5-MTF (Def) & 41.7
        \\
    \ \ T5-MTF (Def+2Pos) & 52.6
        % \\
        % T5-MTF (Prefix)
        % \\
        % T5-MTF (LoRA)
    \\ \midrule
    \multicolumn{2}{l}{\textit{HyperTuning}} \\
    \ \ HyperT5-Prefix (Def) & 36.1
        \\
    \ \ HyperT5-Prefix (Def+2Pos) & 46.6
        \\
    \ \ HyperT5-LoRA (Def) & 35.5
        \\
    \ \ HyperT5-LoRA (Def+2Pos) & 43.6
        \\
        \bottomrule
    \end{tabular}%
    %}
    \caption{
        Results on Super-NaturalInstuctions (S-NI; Test) with T5-XL models.
    }
    \label{tab:table_05_natinst_3b}
}
\end{table}
